Decomposing Counterfactual Explanations for Consequential Decision Making

The goal of algorithmic recourse is to reverse unfavorable decisions (e.g., from loan denial to approval) under automated decision making by suggesting actionable feature changes (e.g., reduce the number of credit cards). To generate low-cost recourse the majority of methods work under the assumption that the features are independently manipulable (IMF). To address the feature dependency issue the recourse problem is usually studied through the causal recourse paradigm. However, it is well known that strong assumptions, as encoded in causal models and structural equations, hinder the applicability of these methods in complex domains where causal dependency structures are ambiguous. In this work, we develop \texttt{DEAR} (DisEntangling Algorithmic Recourse), a novel and practical recourse framework that bridges the gap between the IMF and the strong causal assumptions. \texttt{DEAR} generates recourses by disentangling the latent representation of co-varying features from a subset of promising recourse features to capture the main practical recourse desiderata. Our experiments on real-world data corroborate our theoretically motivated recourse model and highlight our framework's ability to provide reliable, low-cost recourse in the presence of feature dependencies.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec1_introduction.tex <==
Counterfactual explanations provide a means for actionable model explanations at feature level. 
Such explanations, which have become popular among legal and technical communities, provide both an explanation and an instruction: 
the former emphasizes why a certain machine learning (ML) prediction was produced;
the latter gives an instruction on how to act to arrive at a desirable outcome. 

When counterfactual explanations are deployed in systems that involve humans in the loop, feasibility constraints become important. 
Instead of using the term `counterfactual explanations', the term `algorithmic recourse' is often used to highlight precise actions that can be taken by an individual to arrive at a desirable outcome,
%after being subjected to an automated decision
\emph{emphasizing} feasibility constraints that have to be taken into account. 
Those recourses are found by making small changes to an input vector to influence the prediction of a pretrained classifier in a positive way; for example, from ’loan denial' to ’loan approval’, subject to the constraint that an individual's `gender' may not change. 

Several approaches in recent literature tackled the problem of providing recourses by generating counterfactual explanations  \cite{wachter2017counterfactual,ustun2019actionable,karimi2019model,van2019interpretable}. 
For instance, \citet{wachter2017counterfactual} proposed a gradient based approach which finds the nearest counterfactual resulting in the desired prediction. 
\citet{pawelczyk2019} proposed a method which uses a generative model to find recourses in dense regions of the input space.
More recently, \citet{karimi2020intervention} advocated for considering causal structure of the underlying data when generating recourses to avoid spurious explanations. 
These works either assume that the features can be independently manipulated \citep{wachter2017counterfactual}, narrowly focus on manifold constraints \citep{pawelczyk2019} or require a correct specification of the causal graph in combination with the correct structural equation models \citep{karimi2020intervention}.
For example, for many practical use cases, such strong causal assumptions constitute the limiting factor when it comes to the deployment of these recourse methods.

On the other hand, most of the practical approaches implicitly make the \emph{independently manipulable feature} (IMF) assumption.
Therefore, critiques of counterfactual explanations and algorithmic recourse have highlighted the feature dependency issue \cite{barocas2020,Venkatasubramanian2020,Bjorkegren2020manipulation}: in a nutshell, \emph{changing one feature will likely change others}.\footnote{
The terms counterfactual explanations \cite{wachter2017counterfactual}, contrastive explanations \cite{karimi2020survey}, and algorithmic recourse \cite{ustun2019actionable} have been used in similar contexts to refer to similar problems. 
We usually use the term `algorithmic recourse' and refer to \cite{karimi2020survey} for a nuanced discussion of these terms.
}
For instance, a recourse system might ask to increase the feature `income' for a loan approval. 
However, there might be several ways of achieving the same desired outcome of loan approval: either one could increase `income' through a promotion or one could find a new role in a different company. 
In the former case, the value of the variable reflecting `time on job' would go up, which would likely amplify the model's output towards the desirable outcome. 
In the latter case, however, the model's output would likely swing towards a loan rejection, since the short `time on job' opposes the positive influence of the `income' increase (see Figure \ref{fig:correlations_matter}).

\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.49\columnwidth}
\centering
\input{tikz/tikz_correlations_1}
\caption{Possible sparse recourse suggestions ignoring input dependencies.}        
\label{fig:classic_intervention}
\end{subfigure} 
\hfill
\begin{subfigure}[b]{0.49\columnwidth}
\centering
\input{tikz/tikz_correlations_2}
\caption{Recourse can be unreliable, if input dependencies are ignored.}
\end{subfigure}
\caption{Illustrating that input dependencies matter for algorithmic recourse. \textbf{(a)} Most of the algorithmic recourse literature emphasizes the importance of sparse recourses. \textbf{(b)} Recourses optimized for sparsity can be unreliable. We consider an individual who tries to implement a suggested \textcolor{RoyalBlue}{income change} via a \textcolor{BrickRed}{job change} (\textcolor{BlueViolet}{move up and left}) or via a \textcolor{BrickRed}{successful performance review} (\textcolor{PineGreen}{move right and up}). In the upper left, the short `ToJ' is counteracting the positive influence coming from `Income', still leading to a loan rejection. }
\label{fig:correlations_matter}
\end{figure}

For an individual who is subjected to an automated decision system the recourse suggestion is crucial. 
These suggestions, however, can be misleading, especially for approaches that make the IMF assumption, since the omission of feature dependencies comes with the risk that required recourse changes are not reliably captured (see Figure \ref{fig:correlations_matter}).
%To create trust in recourse systems it is therefore important to suggest reliable recourses.
Across different works, various scholars have formulated different requirements on what it means for a recourse suggestion to be reliable. 
We summarize the most important requirements below \citep{wachter2017counterfactual,karimi2019model,keane2020good,joshi2019towards,pawelczyk2019,antoran2020getting,karimi2020intervention,karimi2020probabilistic,verma2020counterfactual}:
\begin{itemize}
\item[(R1)] Recourses should adhere to interdependencies between the input features;
\item[(R2)] Recourses should lie in dense regions of the data distribution;
\item[(R3)] Recourses should be attainable at low cost by the individual;
\item[(R4)] Recourse costs should be controllable by separating important from unimportant features.
\end{itemize}
% To create trust in recourse systems it is therefore important to suggest recourses that reflect the cost of recourse to an individual as reliable as possible. 
% Intuitively, the costs of a counterfactual explanation should reflect the distance between the factual input and the proposed counterfactual vector, thus measuring the changes that need to be made at feature level to achieve the desired outcome. 
%This, however, can be misleading, especially for approaches that make the IMF assumption, since the omission of feature dependencies comes with the risk that required recourse changes are not realistically captured (e.g., Figure \ref{fig:classic_intervention}).
% At the same time, the technical and law literature has opted for explanations that are sparse and seek to change no more than the 'key factors' \citep{barocas2020,wachter2017counterfactual}. This seems to imply a trade-off between the practical cost of recourse and the simplicity of the generated recourse explanations. For example, \citet{pmlr-v124-pawelczyk20a} have empirically and theoretically demonstrated that \emph{independence--based} recourse models generate lower recourse costs than their \emph{manifold--based} counterparts. We will bridge this gap by devising a \emph{dependence--based} recourse model, that captures arbitrary feature correlations, while it entails \emph{independence--based} recourse costs as a special case, if inputs are pairwise independent.
%Another important desideratum is to allow for an interface where the end-users can insert their search preferences over attributes they would like to intervene on. This is crucial since individuals often know best which feature can realistically be changed given their circumstances \citep{barocas2020}. To enable this desideratum for independence-based models, \citet{ustun2019actionable,russell2019efficient,mothilal2020fat} devised different search techniques which allow for targeted feature changes.  Current generative model approaches do not offer control over inputs one wishes to intervene on.
% \textbf{Gjergji: It would be great if we could claim something like this:}
% In this work, we exploit independence between subgroups of features and devise a generative recourse model that captures the main practical desiderata, including flexibility, feasibility, proximity and robustness of interventions. Furthermore, we provide a detailed analysis of the corresponding intervention costs, and show that our approach efficiently and faithfully minimizes the recourse costs. 
Combining requirements R1-R4 in one recourse system poses a severe challenge to making algorithmic recourse practicable in the real world.
In this work, from the perspective of R1, we introduce and address the critical problem of algorithmic recourse in the face of these four challenges.
%We propose a new framework, and study under which conditions it provides strong solutions to our recourse problem. 
More specifically, we make the following key contributions:
\begin{itemize}
\item[(i)] We formulate the problem of algorithmic recourse in the face of data dependencies using generative models (R1, R2).
\item[(ii)] We propose a new framework called \texttt{DEAR} (\textbf{D}is\textbf{E}ntangling \textbf{A}lgorithmic \textbf{R}ecourse) which generates recourses by disentangling the latent representation of co-varying features from a subset of promising recourse features (R1). 
As a byproduct of our framework, we show that recourse actions can be divided into two types of actions: \emph{direct} and \emph{indirect actions}, which can be exploited to lower the cost of recourse (R4).
\item[(iii)] Through theoretical analysis we highlight two aspects. 
First, we show that our framework captures recourse costs by decoupling direct recourse costs from indirect costs. 
The indirect costs result from the \emph{direct} actions and emerge only in the presence of feature dependencies (R1, R2).
Second, we provide recommendations on the choice of direct actions (R4).
\item[(iv)] We conduct extensive experimentation with multiple real-world data sets and various state-of-the-art recourse methods to validate our theoretical analysis, demonstrating the efficacy of our framework.
\end{itemize}
To the best of our knowledge, this work is the first to address R1-R4 using one unifying framework, which will bridge a critical gap in the recourse literature, thereby, paving the way for real-world deployment of algorithmic recourse.

==> sec3_perliminaries.tex <==
In this Section, we discuss the generic formulation leveraged by several state-of-the-art recourse methods including \citep{wachter2017counterfactual}.

\subsection{Algorithmic Recourse: General Formulation} \label{section:background_recourse_independent}
\paragraph{\textbf{Notation}} Before we introduce our framework, we note $\lVert \cdot \rVert$ refers to the 2-norm of a vector, $h(f(\bx))$ denotes the probabilistic output of the trained classifier, where $f: \mathbb{R}^d \to\mathbb{R}$ is a differentiable scoring function (e.g., logit scoring function) and $h: \mathbb{R}\to [0,1]$ is an activation function (e.g., sigmoid) that maps scores to continuous probability outputs. 
We denote the set of outcomes by $y\in \{0,1\}$, where $y=0$ is the undesirable outcome (e.g., loan rejection) and $y=1$ indicates the desirable outcome (e.g., loan approval). 
Moreover, $\hat{y} = \mathbb{I}[h(f(\bx)) > \theta] = \mathbb{I}[f(\bx) > s]$ is the predicted class, where $\mathbb{I}[\cdot]$ denotes the indicator function and $\theta$ is a threshold rule in probability space (e.g., $\theta = 0.5$), with corresponding threshold rule $s$ in scoring space (e.g., $s=0$ when a sigmoid activation is used).

\paragraph{\textbf{The Recourse Formulation}}
Counterfactual explanation methods provide recourses by identifying which attributes to change for reversing an unfavorable model prediction.
While several of these methods incorporate distance metrics (e.g., $\ell_{p}$-norm) or user preferences \citep{rawal2020individualized} to find the desired counterfactuals, some works also impose causal \citep{karimi2020probabilistic} or data manifold constraints \citep{joshi2019towards,pawelczyk2019} to find realistic counterfactuals. 
We now describe the generic formulation leveraged by several state-of-the-art recourse methods.

The goal is to find a set of actionable changes in order to improve the outcomes of instances $\bx$ which are assigned an undesirable prediction under $f$.
Moreover, one typically defines a cost measure in input space $c: \mathbb{R}^d \times \mathbb{R}^d \xrightarrow{} \mathbb{R}_+$. 
Typical choices are the $\ell_1$ or $\ell_2$ norms.
Then the recourse problem is set up as follows:
\begin{align}
    \bdelta^* = \argmin_{\bdelta}  c(\bx, \xC) 
    \text{ s.t. } \xC = \bx + \bdelta, ~ \xC \in \mathcal{A}_d, ~ f(\xC) \geq s.
\label{equation:problem_independent}
\end{align}
The objective in \eqref{equation:problem_independent} seeks to minimize the recourse costs $c(\bx, \xC)$ subject to the constraint that the predicted label $\hat{y}$ flips from $0$ (i.e., $f(\xC) < s$) to $1$ (i.e., $f(\xC) \geq s$), and $\mathcal{A}_d$ represents a set of constraints ensuring that only admissible changes are made to the factual input $x$. 
For example, $\mathcal{A}_d$ could specify that no changes to protected attributes such as `sex' can be made.
The assumption underlying \eqref{equation:problem_independent} is that each feature can be independently manipulated regardless of existing feature dependencies.
Under this so-called independently manipulable feature (IMF) assumption, existing popular approaches use gradient based optimization techniques \citep{wachter2017counterfactual,pawelczyk2021connections}, random search \citep{laugel2017inverse}, or integer programming \citep{ustun2019actionable,karimi2019model,rawal2020individualized} to find recourses.
Although causal recourse methods have been proposed to mitigate this issue, these methods also rely on strong assumptions and require the specification of causal graphical models and corresponding causal structural equations.
In the next Section, we suggest a framework as an alternative to these two lines of work. 

% %\paragraph{Latent Actions are Opaque}
% Using the manifold-based generative recourse models to determine recourse entails two shortcomings. First, recourse is determined by finding latent actions $\bdelta_z$, but these actions neither carry direct meaning nor are they guaranteed to be predictive of the outcome. In fact, if the latent actions correspond to non-discriminative features, then the required changes measured in input space can be large \citep{ortiz2020hold}. Second, end-users have no room to insert their search preferences over inputs they would like to change; a crucial desideratum that independent or causal recourse models allow for \citep{mothilal2020fat,russell2019efficient,ustun2019actionable,karimi2020intervention}.


==> sec4_main_body.tex <==
%So far, we have discussed how recourses generated by existing methods usually ignore input dependencies when generating recourses.
Here, we present our novel recourse framework, \textbf{D}is\textbf{E}ntangling \textbf{A}lgorithmic \textbf{R}ecourse (\texttt{DEAR}), which will fill the gap between the strong causal recourse assumptions and the strong IMF assumption. 
More specifically:
1) We introduce the generative model required to generate recourses under input dependencies (R1, R2),
2) using our model we then show that disentangled representations need to be learned to provide accurate recourse cost estimates (R3),
3) using the disentangled representations we suggest our objective function to find recourses under input dependencies and provide a closed-form expression for the recourses output by our framework (R4) and finally
4) we provide a detailed discussion on how to operationalize and optimize our objective effectively (R4).

\subsection{Our Generative Model and Disentangled Representations}
\paragraph{\textbf{The Generative Model}}
On a high level, our framework consists of separating the latent code of a generative model into (i) observable features $\bx_{\mathcal{S}}$ -- that we wish to perform direct recourse actions on -- and (ii) latent space features $\bv$ that have been trained to become disentangled of the observable features (i.e., $\bv \upmodels \bx_{\mathcal{S}}$). 
A direct recourse action has two effects: a direct effect on the input features that have to be changed, and an indirect effect on other, dependent features. 
The strength of the indirect effect is then determined by a generative model (see Figure \ref{fig:aae}). 
To formalize this intuition, let the input $\bx$ be produced by the following generative model:
\begin{equation}
    \bx = [\bx_{\mathcal{S}}, \bx_{S^c}] = [ g_{\bx_{\mathcal{S}}}(\bv,\bx_{\mathcal{S}}),  g_{\bx_{S^c}} (\bv,\bx_{\mathcal{S}})] = g(\bv, \bx_{\mathcal{S}}),
    \label{eq:generative_model_indepence}
\end{equation}
where $g: \mathbb{R}^k \to \mathbb{R}^d$, $\bv \in \mathbb{R}^{k-|\mathcal{S}|}$ refers to the the latent code and $\bx_{\mathcal{S}}$ corresponds to a subset of the input features where $S \subset  \{1, \dots, d\}$, and the complement set is $S^c = \{1, \dots, d\} ~ \backslash ~ S$. Below we show the importance of disentangled representations for reliable cost estimates.

% KDD
% \begin{figure}[tb]
%          \centering
% \input{tikz/intervention_time}
% \caption{Finding recourse for input $\bx$ with \texttt{DEAR}.
% For an input $\bx$ with $f(\bx) < s$, we encode $[\bx_{\mathcal{S}}, \bv]{=}e(\bx)$. Then, we find direct actions $\textcolor{RoyalBlue}{\bd_{\mathcal{S}}}$, which generate recourse, i.e.\ we find a $\xC$ such that $f(\xC) > s$, where $\xC = [\textcolor{RoyalBlue}{\bd_{\mathcal{S}} } + \bx_{\mathcal{S}},\textcolor{BrickRed}{\check{\bx}_{S^c}}(\bv, \textcolor{RoyalBlue}{\bd_{\mathcal{S}}} + \bx_{\mathcal{S}})]$. The direct action \textcolor{RoyalBlue}{$\bd_{\mathcal{S}}$} has two effects: 1) it changes the features in $\mathcal{S}$ directly (i.e., $\textcolor{RoyalBlue}{\bd_{\mathcal{S}} } + \bx_{\mathcal{S}}$ ), and 2) it changes the features in $\mathcal{S}^c$ indirectly (i.e., $\textcolor{BrickRed}{\check{\bx}_{S^c}}(\bv, \textcolor{RoyalBlue}{\bd_{\mathcal{S}}} + \bx_{\mathcal{S}}))$. The strength of the indirect change $\textcolor{BrickRed}{\check{\bx}_{S^c}}$ is determined by the \text{elasticity of $g_{\bx_{S^c}}$ w.r.t.\  $\bx_{\mathcal{S}}$} (see Proposition \ref{proposition:recourse_costs_ae}).}
% \label{fig:aae}
% \end{figure}


\begin{wrapfigure}{l}{5cm}
\raggedleft
\input{tikz/intervention_time}
\caption{Finding recourse for input $\bx$ with \texttt{DEAR}.
For an input $\bx$ with $f(\bx) < s$, we encode $[\bx_{\mathcal{S}}, \bv]{=}e(\bx)$. Then, we find direct actions $\textcolor{RoyalBlue}{\bd_{\mathcal{S}}}$, which generate recourse, i.e.\ we find a $\xC$ such that $f(\xC) > s$, where $\xC = [\textcolor{RoyalBlue}{\bd_{\mathcal{S}} } + \bx_{\mathcal{S}},\textcolor{BrickRed}{\check{\bx}_{S^c}}(\bv, \textcolor{RoyalBlue}{\bd_{\mathcal{S}}} + \bx_{\mathcal{S}})]$. The direct action \textcolor{RoyalBlue}{$\bd_{\mathcal{S}}$} has two effects: 1) it changes the features in $\mathcal{S}$ directly (i.e., $\textcolor{RoyalBlue}{\bd_{\mathcal{S}} } + \bx_{\mathcal{S}}$ ), and 2) it changes the features in $\mathcal{S}^c$ indirectly (i.e., $\textcolor{BrickRed}{\check{\bx}_{S^c}}(\bv, \textcolor{RoyalBlue}{\bd_{\mathcal{S}}} + \bx_{\mathcal{S}}))$. The strength of the indirect change $\textcolor{BrickRed}{\check{\bx}_{S^c}}$ is determined by the \text{elasticity of $g_{\bx_{S^c}}$ w.r.t.\  $\bx_{\mathcal{S}}$} (see Proposition \ref{proposition:recourse_costs_ae}).}
\label{fig:aae}
\end{wrapfigure}


\paragraph{\textbf{The Importance of Disentanglement Learning}}
Here, we use our generative model from \eqref{eq:generative_model_indepence} and consider recourse cost estimates under this model. 
In the following Proposition, we consider this setting to obtain an intuition on how the generative model required for our framework has to be trained.
%to yield reliable recourse cost estimates. 
\begin{proposition}[Recourse costs]
Under the generative model in \eqref{eq:generative_model_indepence}, the cost of recourse $\lVert \bdelta_x \rVert^2 = \lVert \bx - \xC \rVert^2$ is given by:
\begin{align}
\begin{split}
 \lVert \bdelta_x \rVert^2
 & \approx \underbrace{\bd^\top_{\mathcal{S}} \big( {\bJ_{\bx_{\mathcal{S}}}^{(\bx_{\mathcal{S}})}}^\top {\bJ_{\bx_{\mathcal{S}}}^{(\bx_{\mathcal{S}})}} \big) \bd_{\mathcal{S}}}_{\textcolor{RoyalBlue}{\text{Direct Costs}}} + \underbrace{\bd^\top_{\mathcal{S}} \big({\bJ_{\bx_{\mathcal{S}}}^{(\bx_{S^c})}}^\top \bJ_{\bx_{\mathcal{S}}}^{(\bx_{S^c})}\big) \bd_{\mathcal{S}}}_{\textcolor{BrickRed}{\text{Indirect Costs}}}, \\
where: \\
{\bJ_{\bx_{\mathcal{S}}}^{(\bx_{\mathcal{S}})}} &= \underset{\textcolor{RoyalBlue}{\text{Entanglement costs}}}{\underbrace{\frac{\partial g_{\bx_{\mathcal{S}}}(\bv, \bx_{\mathcal{S}})}{\partial \bv} \frac{\partial \bv}{\partial \bx_{\mathcal{S}}}}} + \underset{\textcolor{RoyalBlue}{\text{Identity Mapping}}}{\underbrace{\frac{\partial g_{\bx_{\mathcal{S}}}(\bv, \bx_{\mathcal{S}})}{\partial\bx_{\mathcal{S}}}}} \\
{\bJ_{\bx_{\mathcal{S}}}^{(\bx_{S^c})}} & = \underset{\textcolor{BrickRed}{\text{Entanglement costs}}}{\underbrace{\frac{\partial g_{\bx_{S^c}}(\bv, \bx_{\mathcal{S}})}{\partial \bv} \frac{\partial \bv}{\partial \bx_{\mathcal{S}}}}} + \underset{\textcolor{BrickRed}{\text{Elasticity of $g_{\bx_{S^c}}$ w.r.t  $\bx_{\mathcal{S}}$}}}{\underbrace{\frac{\partial g_{\bx_{S^c}}(\bv, \bx_{\mathcal{S}})}{\partial \bx_{\mathcal{S}}}}}.
\end{split}
\end{align}
\label{proposition:recourse_costs_ae}
\end{proposition}

The result of Proposition \ref{proposition:recourse_costs_ae} is intuitive.
It says that we can control the recourse costs using the actions $\bd_{\mathcal{S}}$.
We provide the proof in Appendix \ref{appendix:proof_disentanglement}, and make two noteworthy observations.
First, the result reveals that the costs have to be partitioned into \textcolor{RoyalBlue}{direct} and \textcolor{BrickRed}{indirect} costs. 
The direct costs correspond to the costs that one would have obtained from algorithms that use the IMF assumption when searching for recourses (e.g., \citep{wachter2017counterfactual,pawelczyk2021connections,laugel2017inverse,ustun2019actionable,karimi2019model,rawal2020individualized}). 
The indirect costs are due to feature dependencies of $\bx_{\mathcal{S}}$ with $\bx_{S^c}$. 
If $\bx_{\mathcal{S}}$ is independent of $\bx_{S^c}$ (i.e., the elasticity of $g_{\bx_{S^c}}$ w.r.t  $\bx_{\mathcal{S}}$ is $\mathbf{0}$), then a change in $\bx_{\mathcal{S}}$ will not alter $\bx_{S^c}$ and the only cost remaining is the direct cost (we refer to Figure \ref{fig:aae} for a schematic overview of the mechanism). 
Second, we observe that the costs can be \emph{inflated}, if the latent space variables $\bv$ depend on $\bx_{\mathcal{S}}$. 
This is expressed through the \emph{entanglement cost} terms in Proposition \ref{proposition:recourse_costs_ae}. 
To understand how well \texttt{DEAR} does we suggest to track the \emph{entanglement costs} and use them as a quality measure.

\subsection{Our Objective} \label{section:recourse_model}
So far, we have ignored the predictive model $f$ in our considerations. Now, we introduce the predictive model and we rewrite the recourse problem from \eqref{equation:problem_independent} as follows:
\begin{align}
\begin{split}
\bd_{\mathcal{S}}^* &= \argmin_{\bd_{\mathcal{S}}}  c(\bx, \xC ) \\
\text{ s.t. } \xC = g(\bv &,\bx_{\mathcal{S}} + \bd_{\mathcal{S}}), ~ \xC \in \mathcal{A}_d, ~ \bx_{\mathcal{S}} \upmodels \bv, ~
f(\xC) > s,
\end{split}
\label{equation:problem_dependent_partition}
\end{align}
where we have used the insight that $\bx_{\mathcal{S}} \upmodels \bv$ derived from Proposition \ref{proposition:recourse_costs_ae}.
Relative to the objective from \eqref{equation:problem_independent}, our objective in \eqref{equation:problem_dependent_partition} uses our generative model to capture input dependencies. 
Instead of finding recourse actions across the whole input space, we find recourse actions for the inputs in $\mathcal{S}$.
We make recommendation on the choice of $\mathcal{S}$ in the next Section.
Our reformulation has several advantages compared to existing recourse methods from the literature:
i) relative to manifold-based recourse methods \citep{joshi2019towards,pawelczyk2019,mahajan2019preserving,antoran2020getting,Guidotti2019_generative,kenny2020generating,yang2021model} the actions are applied to input space variables as opposed to latent space variables, and thus they are inherently interpretable;
ii) relative to manifold-based recourse methods and recourse methods which use the IMF assumption \cite{wachter2017counterfactual,keane2020good,laugel2017inverse,tolomei2017interpretable,spooner2021counterfactual,karimi2019model,schut2021generating}, we can sharply separate the direct effect, which $\bd_{\mathcal{S}}$ has on $\xC$ via $\bx_{\mathcal{S}}$, from its indirect effect, which $\bd_{\mathcal{S}}$ has on $\xC$ determined by the generative model when it is dependent of $\bx_{S^c}$ (recall Proposition \ref{proposition:recourse_costs_ae});
iii) relative to causal recourse methods \citep{karimi2020intervention,karimi2020probabilistic}, we neither assumed causal graphical models nor did we assume structural equation models to incorporate input dependencies. However, note that the recourses output by our framework cannot be assigned a causal interpretation. We discuss this in Section \ref{section:case_study} using a case-study.

\subsection{A Closed-Form Expression for DEAR's Recourses}
In this Section, we derive an approximate closed-form solution for the objective in \eqref{equation:problem_dependent_partition} which uses our insights from Proposition \ref{proposition:recourse_costs_ae} (i.e., $\bv \upmodels \bx_{\mathcal{S}}$). 
We then use this solution inform the choice of the set $\mathcal{S}$ in the absence of strong prior information or preferences expressed by the end-user. 
Below we provide the closed-form solution.

\begin{proposition}[Recourses by \texttt{DEAR}]
Suppose $\bv \upmodels \bx_{\mathcal{S}}$. Then a first-order approximation $\tilde{\bd}_{\mathcal{S}}^*$ to the optimal recourse $\bd_{\mathcal{S}}^*$ from the objective in \eqref{equation:problem_dependent_partition} using $c=\lVert \bx - \xC \rVert^2$ is given by:
\begin{align}
\bdelta^*_x \approx {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \tilde{\bd}_{\mathcal{S}}^* = \frac{m}{\lambda + \lVert \bw \rVert_2^2} \cdot {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bw,
\label{equation:closed_form_dear}
\end{align}
where $\left.\bY_{\bx_{\mathcal{S}}}^{(\bx)}{:=} \frac{\partial g(\bv, \bx_{\mathcal{S}})}{\partial \bx_{\mathcal{S}} }\right\vert_{\bv=\bv, \bx_{\mathcal{S}}=\bx_{\mathcal{S}}}$, $s$ is the target score in logit space, $m=s{-}f(\bx)$ is the logit gap, $\bw = {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}^\top \nabla f(\bx)$ and $\lambda$ is the trade-off parameter.
\label{proposition:dear}
\end{proposition}

\begin{hproof}
We derive an approximation to the closed-form solution for $\bd_{\mathcal{S}}^*$ by formulating the Lagrangian formulation corresponding to the objective in \eqref{equation:problem_dependent_partition} in its vector quadratic form.
We then use the decoder $g$ to transform the optimal recourse action $\bd_{\mathcal{S}}^*$ to the optimal input space action $\bdelta_{x}^*$.
We refer to Appendix \ref{appendix:proof_closed_form_dear} for the complete proof.
\end{hproof}
The above result is intuitive. The optimal action $\tilde{\bd}_{\mathcal{S}}^*$ applied to the inputs $\bx_{\mathcal{S}}$ is being transformed by the generator Jacobian ${\bY_{\bx_{\mathcal{S}}}^{(\bx)}}$ to yield the optimal action in input space $\bdelta^*_x$. 
The generator Jacobian, in turn, measures the influence that the features in $\mathcal{S}$ have on the input $\bx$. 
%Thus, our first insight is: a sparse generator Jacobian encourages low cost in terms of the 1-norm, $\lVert \bdelta_x^* \rVert_1$. 

In the absence of strong prior information or preferences on which sets of variables $\mathcal{S}$ the actions should be performed, we suggest to use \emph{singletons}, however, $\mathcal{S}$ can also be extended to multiple variables that are thought to form one coherent `concept'.\footnote{
For example, the GMC data set includes 3 variables that describe the `payment morale' of a client: number of times \emph{30 days late}, \emph{60-89 days late} and \emph{more than 90 days late}. 
Thus, $\mathcal{S}$ could include these 3 variables, and our framework allows to analyze to what extent an improvement in the `payment morale' would affect other variables and how the combined change of all these variables would contribute to a change in the prediction. 
}
The insight from Proposition \ref{proposition:dear} becomes more clear, if $\mathcal{S}$ are singletons.
Then, $\bw$ from  \eqref{equation:closed_form_dear} becomes a scalar.
Therefore, to make most progress towards the desired outcome at first order, $\bY_{\bx_{\mathcal{S}}}^{(\bx)}$ should have a high similarity to the model gradient $\nabla f(\bx)$ in the dot-product sense. 
To see this, consider a first-order approximation of $f(\bx + \bdelta^*_x) \approx f(\bx) + \nabla f(\bx)^\top \bdelta^*_x  = f(\bx) + \frac{m \cdot w}{\lambda + \lVert \bw \rVert_2^2} \cdot  \nabla f(\bx)^\top \bY_{\bx_{\mathcal{S}}}^{(\bx)}$.
To push the score of $f(\bx)$ towards the target score $s\geq 0$, $\mathcal{S}$ should be chosen such that the dot product $\nabla f(\bx)^\top \bY_{\bx_{\mathcal{S}}}^{(\bx)}$ is high.
In other words, i) the feature from $\mathcal{S}$ ideally has high discriminative power with respect to the predictive model $f$, and ii) the feature from $\mathcal{S}$ should influence other features from $\mathcal{S}^c$ that have high discriminative power, too.
In the absence of strong prior information on which variables to perform the direct actions, it seems natural to use a local attribution method (e.g., \citep{lundberg2017unified}) to determine feature relevance.
In the next Section, we present an algorithmic procedure that allows us to compute minimal cost recourses under feature dependencies.

\subsection{Optimizing our Objective} \label{section:marie_algorithm}
Motivated by the insights from Propositions \ref{proposition:recourse_costs_ae} and \ref{proposition:dear}, we present an algorithmic procedure to compute minimal cost recourses under feature dependencies using a penalty term during autoencoder training that encourages disentanglement of $\bx_{\mathcal{S}}$ and $\bv$ in order to keep the \emph{entanglement costs} low.
In summary, \texttt{DEAR} requires two steps: first, we need to obtain a latent space representation $\bv$, which is independent of $\bx_{\mathcal{S}}$. 
Second, we require an optimization procedure to identify the nearest counterfactual.

\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.49\columnwidth}
\centering
\input{tikz/training_time}
\caption{Conditional autoencoder}        
\label{fig:c_ae}
\end{subfigure} 
\hfill
\begin{subfigure}[b]{0.49\columnwidth}
\centering 
\input{tikz/resnet}
\caption{\texttt{ResNet} component within the decoder}
\end{subfigure}
\caption{\texttt{DEAR}'s autoencoder architecture.
In (a), we show our conditional autoencoder architecture, which we train subject to the Hessian penalty described in Section \ref{section:marie_algorithm}. 
In (b), we show how we achieve the identity mapping between $\bx_{\mathcal{S}}$ and the reconstructed $\bx^r_{\mathcal{S}}$ using a \texttt{ResNet} component \citep{he2016deep,he2016identity}: we add $\bx_{\mathcal{S}}$ to $\bx^r_{\mathcal{S}}$  before passing the arguments to the loss $\mathcal{L}_R$ from \eqref{eq:reconstruction_loss}.}
\label{figure:architecture}
\end{figure}

\paragraph{\textbf{Step 1: Training the Generative Model}}
The main idea is to train a generative model, in which $\bx_{\mathcal{S}}$ is independent of the latent variable $\bv$, while providing high-quality reconstruction of the input $\bx$.
Thus, the training loss for the generative model consists of two components. 
First, it consists of both an encoder network $e$ and decoder network $g$, for which the reconstruction loss,
\begin{align}
\mathcal{L}_R(g,e; \bx_{\mathcal{S}}) =\lVert g( e(\bx), \bx_{\mathcal{S}}) - \bx \rVert_2^2,
\label{eq:reconstruction_loss}
\end{align}
guides both networks towards a good reconstruction of $\bx$.
Second, we want to drive the \emph{entanglement costs} to 0, for which we need the decoder $g$ to be disentangled with respect to the latent space, i.e., each component of $\bz = [\bv, \bx_{\mathcal{S}}]$ should ideally control a single factor of variation in the output of $g$. 
To formalize this intuition, recall that $g(\bx_{\mathcal{S}}, \bv) = \bx \in \mathbb{R}^d$, where each output $g_j=x_j$ for $1 \leq j \leq d$ has its own $|\bx_{\mathcal{S}}| \times |\bv|$ Hessian matrix $\bH^{(j)}$. 
We refer to the collections of the $d$ Hessian matrices as $\bH$.
Thus, the second loss we seek to minimize is given by:
\begin{align}
    \mathcal{L}_{\bH}(g; \bx_{\mathcal{S}}) = \sum_{j=1}^d \bigg( \sum_{k=1}^{|\bv|} \sum_{l=1}^{|\bx_{\mathcal{S}}|} H_{kl}^{(j)} \bigg),
\label{eq:hessian_penalty}
\end{align}
which is also known as the Hessian penalty \citep{peebles2020hessian}.
We illustrate the intuition of this objective on the $j$-th output $x_j$: we regularize the Hessian matrix $\bH^{(j)} = \frac{\partial}{\partial \bv} \frac{\partial g_j}{\partial \bx_{\mathcal{S}}}$ and encourage its off-diagonal terms to become $0$. 
Driving the off-diagonal terms to $0$ implies that $\frac{\partial g_j}{\partial \bx_{\mathcal{S}}}$ is not a function of $\bv$ and thus $\bv$ plays no role for the output of $g_j$ when searching for minimum cost actions using $\bx_{\mathcal{S}}$.
We use the Hessian penalty from \citep{peebles2020hessian} in our implementation.
%Third, to keep the cost of recourse low we use the $\ell_1$-norm of the jacobian as a regularizer, i.e., we add $\lVert {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}\rVert_1$ to the loss.
Finally, Proposition \ref{proposition:recourse_costs_ae} requires the identity mapping between the latent space $\bx_{\mathcal{S}}$ and the reconstructed $\bx^r_{\mathcal{S}}$.
We encourage our generator $g$ to learn this mapping by using a \texttt{ResNet} architecture \citep{he2016deep,he2016identity} as shown in Figure \ref{figure:architecture}.

\paragraph{\textbf{Step 2: Finding Minimal Cost Actions $\bd_{\mathcal{S}}$}} Given our trained generative model from step 1, we rewrite the problem in \eqref{equation:problem_dependent_partition} using a Lagrangian with trade-off parameter $\lambda$. 
For a given encoded input instance $e(\bx) = [\bv, \bx_{\mathcal{S}}]$, our objective function reads:
\begin{align}
     \bd^*_{\mathcal{S}} = \argmin_{\bd_{\mathcal{S}}, ~ \xC \in \mathcal{A}_d} \mathcal{L}  = \argmin_{\bd_{\mathcal{S}}, ~ \xC \in \mathcal{A}_d} \ell\big(f(\xC(\bd_{\mathcal{S}})), s \big) + \lambda \lVert \bx - \xC(\bd_{\mathcal{S}}) \lVert_1 ,
\label{equation:surrogate_loss_dear}
\end{align}
where $\xC(\bd_{\mathcal{S}}) = g(\bv, \bx_{\mathcal{S}}+\bd_{\mathcal{S}})$ is a potential counterfactual in input space, $\ell(\cdot, \cdot)$ denotes the MSE loss, and $s\geq0$ is the target score in logit space. 
% The MSE loss encourages the model output $f(\xC(\bd_{\mathcal{S}}))$ to be pushed to the target logit score $s$. 
The term on the right side encourages the counterfactual $g(\bv, \bx_{\mathcal{S}}+\bd_{\mathcal{S}}) = \xC$ to be close to the given input point $\bx$, while the left hand side encourages the predictions to be pushed from the factual output $f(\bx)$ towards s. 
We do gradient descent iteratively on the loss function in \eqref{equation:surrogate_loss_dear} until the class label changes from $y=0$ to $y=1$.
Algorithm \ref{algorithm:dear_differentiable} summarizes our optimization procedure.
Below we further discuss how other constraints can be included into our objective.
\begin{algorithm}[tb]
   \caption{\texttt{DEAR}}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} $f$, $\bx$ s.t.\ $f(\bx){<}0$, $g$, $e$, $\lambda> 0$, Learning rate: $\alpha>0$, $s\geq 0$, $\mathcal{S}$
   \STATE {\bfseries Initialize:} $\bd_{\mathcal{S}} = \mathbf{0}$, $ e(\bx)=[\bv, \bx_{\mathcal{S}}]$, $\xC = g(\bv, \bx_{\mathcal{S}} + \bd_{\mathcal{S}})$
   \WHILE{$f(\xC)< s$} 
   \STATE $\bd_{\mathcal{S}} =  \bd_{\mathcal{S}} - \alpha \cdot \nabla_{\bd_{\mathcal{S}}} \mathcal{L}(\xC(\bd_{\mathcal{S}});f, s, \lambda)$ \COMMENT{Optimize
   \eqref{equation:surrogate_loss_dear}}
   \STATE $\xC = g(\bv, \bx_{\mathcal{S}}+\bd_{\mathcal{S}})$
   \ENDWHILE ~ \COMMENT{Class changed, i.e., $f(\xC) \geq s$}
   \STATE {\bfseries Return:} $\xC^* = \xC$ 
\end{algorithmic}
\label{algorithm:dear_differentiable}
\end{algorithm}

==> sec5_experiments.tex <==
\paragraph{\textbf{Encoding Monotonicity Constraints}}
In the presence of strong prior knowledge on how certain features are allowed to change (e.g., `years of schooling' (yos) or `age' can only go up) one can add Hinge-losses \citep{mahajan2019preserving} to encourage monotonicity constraints.
Let $x_{yos}$ correspond to the schooling feature. Then we can add $- \min(0, \check{x}_{yos} - x_{yos})$ to the loss function in \eqref{equation:surrogate_loss_dear} to ensure that the counterfactual $\check{x}_{yos}$ should increase, where $\check{x}_{yos}$ is the corresponding entry from $g(\bv, \bx_S+\bd_{\mathcal{S}})$. 
%In Appendix \ref{Appendix:architecture_params}, we discuss how we set the constraints on each of the features.

\paragraph{\textbf{Handling Categorical Variables}}
Using \texttt{DEAR}, one can easily handle (high-cardinality) categorical features. We can turn all categorical features into numeric features by standard one-hot encoding. For each categorical feature, we can then use a softmax-layer after the final output layer of the decoder. 
For the purpose of the one-hot-encoded reconstruction, we apply the argmax.

%\paragraph{\textbf{On the Choice of $\mathcal{S}$}}
%In the absence of strong prior information on which variables to perform the direct actions, it is natural to leverage the insight from Proposition \ref{proposition:dear} and use a local attribution method (e.g., \citep{lundberg2017unified}) to determine feature relevance.
%In our experiments, we consider the 5 most relevant features for an instance.

\begin{figure*}[tb]
\centering
\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=\textwidth]{images/cost_comparisons_f_Adult_both.pdf}
\caption{Adult}
\label{fig:adult_cost_comparison}
\end{subfigure}
\vfill
\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=\textwidth]{images/cost_comparisons_f_COMPAS_both.pdf}
\caption{COMPAS}
\label{fig:compas_cost_comparison}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=\textwidth]{images/cost_comparisons_f_Give_Me_Some_Credit_both.pdf}
\caption{Give Me Credit}
\label{fig:gmc_cost_comparison}
\end{subfigure}
\caption{Measuring the cost of algorithmic recourse across different recourse methods using the $\ell_1$ cost. 
We use boxplots to show the distribution of recourse costs across all individuals from the test set who require algorithmic recourse. 
The numbers above the maximum values correspond to the white dots (= median recourse costs). 
The color of the boxplots represent the type of the recourse method: The methods with `I' use the IMF assumption, the methods with `M' purely focus on the data manifold constraints, and methods with `G' use a graphical model to generate recourses through dense paths. `D' refers to our method which takes both manifold and input dependencies into account.
Section \ref{section:experiment_evaluation} provides a detailed discussion of the results.}
\label{fig:cost_results}
\end{figure*}



\section{EXPERIMENTAL RESULTS}\label{section:experiments}
In this Section, we conduct extensive quantitative and qualitative evaluations to analyze \texttt{DEAR}'s performance using our conceptual insights from the previous Section.
Quantitatively, we conduct a \emph{baseline comparison} contrasting our framework \texttt{DEAR} with state-of-the-art recourse methods \citep{pawelczyk2021carla} using common evaluation measures from the recourse literature such as recourse costs and reliability measures.
Qualitatively, we consider three aspects: (i) the \emph{entanglement costs}, (ii) the structure of the \emph{cost splits} (i.e., direct vs.\ indirect costs) and (iii) a \emph{case study} to showcase the advantages of our new framework. 

\definecolor{Gray}{gray}{0.9}
\begin{table*}[tb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccccccccccccccc}
\toprule
&&
\multicolumn{6}{c}{Adult} & \multicolumn{6}{c}{COMPAS}  & \multicolumn{6}{c}{GMC}  \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14} \cmidrule(lr){15-20}
&& \multicolumn{3}{c}{LR} & \multicolumn{3}{c}{ANN} & \multicolumn{3}{c}{LR} & \multicolumn{3}{c}{ANN} & \multicolumn{3}{c}{LR} & \multicolumn{3}{c}{ANN} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17} \cmidrule(lr){18-20}
\multicolumn{2}{c}{Method} & SR ($\uparrow$) & CV ($\downarrow$) & YNN ($\uparrow$) & SR ($\uparrow$) & CV ($\downarrow$) & YNN ($\uparrow$) & SR ($\uparrow$) & CV ($\downarrow$) & YNN ($\uparrow$) & SR ($\uparrow$) & CV ($\downarrow$) & YNN ($\uparrow$) & SR ($\uparrow$) & CV ($\downarrow$) & YNN ($\uparrow$) & SR ($\uparrow$) & CV ($\downarrow$) & YNN ($\uparrow$) \\
\cmidrule(lr){1-2} 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
\cmidrule(lr){15-17} \cmidrule(lr){18-20}
\multirow{2}{*}{I} & \texttt{GS} &\textbf{1.00}	& \textbf{0.00}	&0.55	&\textbf{1.00}	& \textbf{0.00}	&0.34	&\textbf{1.00}	& \textbf{0.00}	&0.93	&\textbf{1.00}	& \textbf{0.00}	&0.99	&\textbf{1.00}	& NA	&0.19	&\textbf{1.00}	& NA	&0.64 \\
& \texttt{SCFE} &0.73	& \textbf{0.00}	&0.81	&0.84	& \textbf{0.00}	&0.67	&0.08	& \textbf{0.00}	&0.91	&0.92	& \textbf{0.00}	&0.97	&\textbf{1.00}	& NA	&0.23	&0.98	& NA	&0.65 \\
\midrule
\multirow{2}{*}{M} &\texttt{REVISE} & 0.35	& \textbf{0.00}	& 0.37	&\textbf{1.00}	& 0.12	&\textbf{0.72}	&0.63	& 0.11	&\textbf{1.00}	& 0.99	& 0.12 	& 0.98	&0.99	& NA	&\textbf{\textbf{1.00}}	&\textbf{\textbf{1.00}}	& NA	&0.95 \\
&\texttt{CCHVAE} &0.54	& 0.17	&0.53	&\textbf{1.00}	& 0.07	&0.61	&\textbf{1.00}	& 0.32	&\textbf{1.00}	&\textbf{1.00}	& 0.17	&0.96	&\textbf{1.00}	& NA	&0.24	&\textbf{1.00}	& NA	&0.80 \\
\midrule
\multirow{2}{*}{G} &\texttt{FACE-K} & 0.99	& 0.36	&0.71	&\textbf{1.00}	& 0.29	&0.57	&0.99	& 0.38	&\textbf{1.00}	&0.60	& 0.40	&\textbf{\textbf{1.00}}	&\textbf{\textbf{1.00}}	& NA	& 0.95	&\textbf{1.00}	& NA	& 0.96 \\
&\texttt{FACE-E} &0.74	& 0.38 &0.70	&0.99	& 0.30	&0.58	&0.99	& 0.41	&\textbf{1.00}	&0.39	& 0.40	&\textbf{1.00}	&\textbf{1.00}	& NA	&0.94	&\textbf{1.00}	& NA	&\textbf{0.97} \\
\rowcolor{Gray}
\midrule
D &\texttt{DEAR} & \textbf{1.00}	& \textbf{0.00} 	& \textbf{0.84}	& \textbf{1.00}	& \textbf{0.00}	& 0.70	&\textbf{1.00}	& \textbf{0.00}	&\textbf{1.00}	&\textbf{1.00}	& 0.01	&\textbf{1.00}	&\textbf{1.00}	& NA	&0.91	&\textbf{1.00}	& NA	&0.94
   \\
\bottomrule
\end{tabular}%
}
\caption{Measuring the reliability of algorithmic recourse for the ANN and LR models on all data sets. The \emph{success rate} (SR), \emph{constraint violation} (CV) and \emph{$y$-nearest neighbors} (YNN) measures are described in Section \ref{section:experiments}. For GMC, there were no immutable features and therefore we are reporting NA. 
Our method (i.e., \texttt{DEAR}) usually performs on par or better relative to other recourse methods.}
\label{tab:reliability}
\end{table*}

\begin{figure*}[tb]
\centering
\begin{subfigure}[b]{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{images/ent_error_Adult_f.pdf}
\caption{Adult}
\label{fig:error_adult}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{images/ent_error_COMPAS_f.pdf}
\caption{COMPAS}
\label{fig:error_compas}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{images/ent_error_GMC_f.pdf}
\caption{GMC}
\label{fig:error_gmc}
\end{subfigure}
\caption{Evaluating \texttt{DEAR}'s entanglement costs on all data sets. 
At the end of autoencoder training, we compute the Hessians' off-diagonal elements of the decoder and average them (see Section \ref{section:experimen_details} for more details). 
We then plot these averaged values using boxplots across test instances.
The feature names indicate the sets $\mathcal{S}$, that we perform direct recourse actions on. 
The white dots indicate the median entanglement costs, and the box indicates the interquartile range.
In line with Proposition \ref{proposition:recourse_costs_ae}, the costs are pushed to $0$.
}
\label{fig:dis_error_prop1}
\end{figure*}


\subsection{Details on Experiments}\label{section:experimen_details}

\paragraph{\textbf{Real--world Data}} Our first data set is the \emph{Adult} data set taken from the UCI repository. This data set consists of approximately $48K$ samples with demographic (e.g., race, sex), education and employment (e.g., degree, occupation, hours-per-week), personal (e.g., marital status, relationship), financial (capital gain/loss) features where the label predicts whether an individual's income exceeds $50K\$$ per year ($y=1$). 
Our second data set, \emph{COMPAS} (Correctional Offender Management Profiling for Alternative Sanctions) consists of defendants' criminal history, jail and prison time, demographics and the goal is to predict recidivism risk for defendants from Broward County, Florida.
Our third data set is the \emph{Give Me Credit} data set from 2011 Kaggle competition.
It is is a credit scoring data set, consisting of 150,000 observations and 11 features. 
The classification task consists of deciding whether an instance will experience financial distress within the next two years (\textit{SeriousDlqin2yrs} is 0). %or not.

\textbf{Prediction Models} For all our experiments, we obtain counterfactual explanations for two classification models, for which we provide additional details in Appendix \ref{Appendix:architecture_params}:
\begin{itemize}
\item[LR:] Logistic regression: This is a binary classifier that was trained without regularization.
\item[ANN:] Artificial Neural Network: This is binary classifier with a two-layer network that was trained with ReLU activation functions.
\end{itemize}

\textbf{Recourse Methods}
For all data sets, recourses are generated in order to flip the prediction label from the unfavorable class ($y = 0$) to the favorable class ($y = 1$). 
We partition the data set into 80-20 train-test splits, and do the model training and testing on these splits. 
We used the recourse implementations from the open-source library \texttt{CARLA} \citep{pawelczyk2021carla} to generate recourses.
The library includes state-of-the-art recourse methods. 
We use the following six methods as our baselines for comparison: 
\begin{itemize}
    \item[I:] \texttt{GS} \citep{laugel2017inverse}: Under the \emph{IMF assumption}, this is a classifier-agnostic method that generates recourses by conducting random search in input space.
    \item[I:] \texttt{SCFE} \citep{wachter2017counterfactual}: Under the \emph{IMF assumption}, this method generates recourses by solving a variant of \eqref{equation:problem_independent} using iterative gradient descent.
    \item[M:] \texttt{REVISE} \citep{joshi2019towards}: To find recourses that lie on the \emph{data manifold}, this method utilizes a trained autoencoder to transform the input space into a latent embedding space. \texttt{REVISE} then uses gradient descent in latent space to find recourses that lie on the data manifold.
    \item[M:] \texttt{CCHVAE} \citep{pawelczyk2019}: This is a classifier-agnostic method to find recourses that lie on the \emph{data manifold}. \texttt{CCHVAE} also uses a trained autoencoder to transform the input space into a latent embedding space. The latent representation is then randomly perturbed to find recourses.
    \item[G:] \texttt{FACE-K} \& \texttt{FACE-E} \citep{Poyiadzi2020}: This is classifier-agnostic method that finds recourses that lie on paths along dense regions. These methods construct \emph{neighbourhood graphs} to find paths through dense regions. The graph is either an $\epsilon$-graph (FACE-E) or a $k$-nearest neighbour graph (FACE-K).
\end{itemize}
Note that `I' abbreviates methods which use the IMF assumption, `M' abbreviates methods which generate recourses that lie on the data manifold, and `G' abbreviates methods, which use a graphical model to generate recourses that lead through dense paths. `D' refers to our method (i.e., \texttt{DEAR}), which takes input dependencies into account.
To allow for a fair comparison across the explanation models, which use autoencoders, we use similar base architectures for \texttt{DEAR}.
Appendix \ref{Appendix:architecture_params} provides implementation details for the recourse methods and of all used autoencoder models. 
We compute all evaluation measures by using the min-max normalized inputs used for training the classification and generative models. 
Below we describe the evaluation measures.

% \begin{figure}
% \centering
% \begin{subfigure}[b]{\columnwidth}
% \includegraphics[width=\columnwidth]{images/Feature_PairsAdult_Artificial Neural Network.pdf}
% \caption{Adult}
% \label{fig:pairs_adult}
% \end{subfigure}
% \vfill
% \begin{subfigure}[b]{\columnwidth}
% \includegraphics[width=\columnwidth]{images/Feature_PairsGive_Me_Some_Credit_Artificial Neural Network.pdf}
% \caption{GMC}
% \label{fig:pairs_gmc}
% \end{subfigure}
% \caption{Relative frequency of important feature pairs that need to change for the ANN model. Associated with each identified minimum cost intervention, we plot the second most important feature that should be changed together with the intervention feature from $\mathcal{S}$. For example, changing the capital loss would go hand in hand with a change in the years of education.}
% \label{fig:pairs}
% \end{figure}

\paragraph{\textbf{Recourse Costs}}
Since we are interested in generating small cost recourses, we define a notion of distance from the counterfactual explanation to the input point. 
As all methods under consideration minimize the $\ell_1$ norm, we use this measure and compare the $\ell_1$-costs across the methods. 

\paragraph{\textbf{Entanglement Costs}}
For a fixed set $\mathcal{S}$, for every instance at the end of training, we obtain $d$ Hessian matrices $\bH^{(j)} = \frac{\partial^2 g}{\partial \bv \partial x_S}$ for $1 \leq j \leq d$.
We then average the Hessian off-diagonal elements across all $j$ and plot their distribution across all training instances.
We can only do this for our recourse method \texttt{DEAR}.

\paragraph{\textbf{Constraint Violations (CV)}}
We set the protected attributes `sex' and `race' to be immutable for the Adult and COMPAS data sets, and count how often each of the explanation models suggests changes to these protected features. 
GMC has no protected attribute.

\paragraph{\textbf{Label Neighborhood (YNN)}}
 We also use a measure that evaluates how much data support recourses have from positively classified instances \citep{pawelczyk2021carla}.
 Ideally, recourses should be close to correct positively classified individuals, which is a desideratum formulated by the authors of \citep{laugel2019dangers}.
 Values of \text{YNN} close to 1 imply that the neighbourhoods around the recourses consists of points with the same predicted label, indicating that the neighborhoods around these points have already been reached by positively classified instances.
% \begin{equation}
% \text{yNN} = 1 - \frac{1}{Nk} \sum_{i \in \check{H}^-}^N \sum_{j \in \text{kNN}(\xC_i)} \big|f_b(\xC_i) - f_b(x_{j})\big|,  \label{eq:measure2}
% \end{equation}
% where kNN denotes the $k$-nearest neighbours of $x$, and $f_b(x) = \mathbb{I}[f(x) > 0.5]$ is the binarized classifier. Values of \text{yNN} close to 1 imply that the neighbourhoods around the counterfactual explanations consists of points with the same predicted label, indicating that the neighborhoods around these points have already been reached by positively classified instances. We use a value of $k:=5$, which ensures sufficient data support from the positive class.

\paragraph{\textbf{Success Rate (SR)}} Some generated recoures do not alter the predicted label of the instance as anticipated. 
We keep track of how often the suggested counterfactual yield successful recourse by counting the fraction of the respective methods' correctly determined counterfactuals.

\subsection{Evaluation} \label{section:experiment_evaluation}
\paragraph{\textbf{Recourse Costs}} 
The baseline comparisons regarding the cost of recourse are shown in Figure \ref{fig:cost_results}.
Relative to methods that use the IMF assumption (i.e., \texttt{GS}, \texttt{SCFE}), \texttt{DEAR}'s median costs are higher. 
This is to be expected since \texttt{SCFE} and \texttt{GS} \emph{ignore feature dependencies}, essentially providing a lower bound for \texttt{DEAR}'s recourse costs.
Relative to manifold-based recourse methods (i.e, \texttt{REVISE} and \texttt{CCHVAE}), \texttt{DEAR} usually performs more favourably ensuring up to 50 percent less costly median recourse costs. 
This is due to the fact that \texttt{DEAR} can use the most discriminative features in input space -- as opposed to latent space -- to search for recourses. 
Relative to the graph-based methods (i.e., \texttt{FACE-K} and \texttt{FACE-E}) our method performs significantly better.
Since \texttt{FACE} has to ensure connected paths, their costs are usually the highest.

\begin{figure}[tb]
\centering
\begin{subfigure}[b]{0.49\columnwidth}
\centering
\includegraphics[scale=0.32]{images/Cost_Splits_all_Linear.pdf}
\label{fig:cost_split_linear}
\caption{Logistic Regression}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\columnwidth}
\centering
\includegraphics[scale=0.32]{images/Cost_Splits_all_ANN.pdf}
\caption{Artificial Neural Network}
\label{fig:cost_split_ann}
\end{subfigure}
\caption{Cost splits as suggested by Proposition \ref{proposition:recourse_costs_ae} on both classifiers across all data sets.
The \textcolor{RoyalBlue}{direct costs} corresponds to the direct action \textcolor{RoyalBlue}{$\bd_{\mathcal{S}}$} and are measured as $\lVert \textcolor{RoyalBlue}{\bd_{\mathcal{S}}} \rVert_1$. 
The \textcolor{BrickRed}{indirect costs} are measured as $\lVert \bx_{S^c} -  \textcolor{BrickRed}{\check{\bx}_{S^c}}(\bv, \textcolor{RoyalBlue}{\bd_{\mathcal{S}}} + \bx_S) \rVert_1$.
}
\label{fig:cost_splits}
\end{figure}


\paragraph{\textbf{Reliability of Recourse}}
We measure the reliability of recourse using SR, CV and YNN presented in the previous Section. The results across all methods, data sets and classifiers are shown in Table \ref{tab:reliability}.
We see that \texttt{DEAR} has the highest SRs across all data sets and classifiers, among the highest YNN scores, and one of the lowest constraint violation rates. 
Compared to the manifold-based recourse methods, \texttt{DEAR}'s success rate is up to 45 percentage points higher. 
This is due to the fact that the lower dimensional data manifold can end before the decision boundary is reached and thus the manifold-based methods, which search for recourse in latent space, sometimes get stuck before they find a counterfactual instance (see \citep{downs2020interpretable} for a detailed analysis of this phenomenon). 
\citet[Appendix]{antoran2020getting} report a similar finding. 
A similar reason probably prevents FACE from reaching high SRs.
Our model does not suffer from this shortcoming since it primarily uses the most discriminative features in input space (Proposition \ref{proposition:dear}) to search for recourses, resulting in SRs of $1$.

\paragraph{\textbf{Qualitative Analysis}}
Finally, we analyze our recourse model qualitatively. 
We start by analyzing the \emph{entanglement costs}. 
As required by Proposition \ref{proposition:recourse_costs_ae}, we require these costs to be pushed to 0. 
We plot the distribution of the averaged off-diagonal terms in Figure \ref{fig:dis_error_prop1}. 
The results show that the entanglement cost is consistently pushed to 0 (most medians are at 0). The only exception occurs for the feature `workclass' for which our autoencoder network performs less well at concentrating the costs at 0 (right bar in the left panel). 
In summary, however, our mechanism is very well aligned with Proposition \ref{proposition:recourse_costs_ae}'s requirement of disentangled $\bv$ and $\bx_S$.

% \begin{table}[tb]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrccc}
% \toprule
% & & \multicolumn{3}{c}{Explanation Model} \\
% \cmidrule(lr){3-5}
% \multicolumn{2}{c}{Factual} & \texttt{SCFE} (\ref{equation:problem_independent}) & \texttt{REVISE} (\ref{equation:problem_dependent}) & \texttt{DEAR} (\ref{equation:problem_dependent_partition}) \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){3-3}
% \cmidrule(lr){4-4}
% \cmidrule(lr){5-5}
% \texttt{Age} & 45 & \textbf{58} & 45 & \textcolor{BrickRed}{\textbf{48}}  \\
% \texttt{Educ} & 9 & \textbf{7} & \textbf{11} & 9 \\
% \texttt{C-gain} & 0 & 0 & \textbf{2110} & \textcolor{BrickRed}{\textbf{307}} \\
% \texttt{Hours} & 0 & 0 & \textbf{80} & \textcolor{BrickRed}{\textbf{24}} \\
% \texttt{C-loss} & 60 & \textbf{20} & \textbf{45} & \textcolor{RoyalBlue}{\textbf{41}} \\
% \texttt{W-class} & Private: No & No & No &No \\
% \texttt{M-status} & Married: No & No & No & No \\
% \texttt{Occu} & Specialized: No & No & \textbf{Yes} & \textcolor{BrickRed}{\textbf{Yes}} \\
% \texttt{Race} & White: No & No& No& No\\
% \texttt{Sex} & Male: No  & No & No &No \\
% \texttt{Native} & US: Yes & Yes & Yes & Yes \\
% \midrule
% ANN & $>50K$: No & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Comparing recourses qualitatively across explanation methods for a factual instance. The bottom row shows the ANN classifier's predicted class outcomes. For \texttt{DEAR}, the recourse intervention was done to \textcolor{RoyalBlue}{\texttt{C-loss}}. The remaining features changed as a result of this. For \texttt{CCHVAE}, the results were similar to those by \texttt{REVISE}. We discuss the results in Section \ref{section:experiments}.}
% \label{tab:typical_example}
% \end{table}

\subsection{Case Study: Credit Risk}\label{section:case_study}
As a practical example, we showcase additional insights that our recourse model can provide.
%We particularly focus on the Give Me Credit data set.
First, we analyze the cost splits.
According to Proposition \ref{proposition:recourse_costs_ae}, we can split the costs of recourse into a direct and an indirect component.
We show these cost splits in Figure \ref{fig:cost_splits} verifying that the elasticity of $g_{\bx_{S^c}}$ w.r.t.\ $\bx_{\mathcal{S}}$ is non-zero, i.e., we observe a strong presence of feature dependencies. 
Next, we analyze the cost splits from a semantic point of view.
In Figure \ref{fig:cost_splits_gmc}, we show the distribution of important feature pairs that need to change together to lead to loan approvals for individuals from the \emph{Give Me Credit} data set: 
the x-axis shows the direct actions resulting in the lowest costs, and the y-axis shows the relative frequency of the most important indirect actions.
The following noteworthy patterns emerge: 
(i) the non-linear classifier has picked up more non-linear relations since the the feature, on which the minimum cost direct actions are suggested, vary more heavily across instances for the ANN model (bottom panel) relative to the LR model (top panel); 
(ii) we see intuitive patterns emerge. 
For example, a decrease in `revolving utilization' is often followed by a decrease in the number of `loans', which is semantically meaningful suggesting ways to reduce the `revolving utilization'.
Finally, we emphasize that our method showcases the importance of feature dependencies for reliable algorithmic recourse by highlighting how it arrived at the recourse.
The recourses output by our framework should not be mistaken for causal recourses.

\begin{figure}[tb]
\centering
\begin{subfigure}[b]{\columnwidth}
\centering
\includegraphics[width=\columnwidth]{images/Feature_Pairs_fGive_Me_Some_Credit_Linear.pdf}
\caption{Logistic Regression}
\label{fig:cost_split_gmc_lr}
\end{subfigure}
\vfill
\begin{subfigure}[b]{\columnwidth}
\centering
\includegraphics[width=\columnwidth]{images/Feature_Pairs_fGive_Me_Some_Credit_ANN.pdf}
\caption{Artificial Neural Network}
\label{fig:cost_split_gmc_ann}
\end{subfigure}
\caption{We show the rel.\ frequency of important feature pairs that need to be changed together.
Associated with each direct minimum cost action on the x-axis (i.e., $\bd_{\mathcal{S}}$), we plot the second most important feature (y-axis) that should change together with the direct action feature from $\mathcal{S}$.
For example, in the bottom panel, for 10 percent of all instances, decreasing '60-89 days late' goes hand in hand with either a decrease in '30-60 days late' or a decrease in 'more than 90 days late'.}
\label{fig:cost_splits_gmc}
\end{figure}

==> secApp.tex <==
%\raggedtop
%\section*{Appendix Summary} 
% Section \ref{appendix:proof} provides a detailed proof of Proposition \ref{proposition:recourse_costs_marie}. Section \ref{app:add_experiments} presents the remaining experiments we referred to in the main text.
% Finally, in Section \ref{Appendix:architecture_params}, we provide implementation details for all models used in our experiments including (i) the supervised learning models, (ii) the involved recourse methods, and the (iii) generative models required to run the manifold-based methods.
\section{Theoretical Analysis} \label{appendix:proof}
\subsection{Proof of Proposition \ref{proposition:recourse_costs_ae}} \label{appendix:proof_disentanglement}
\emph{Proof}(Recourse Costs by \texttt{DEAR})
First, we note that $\bv$ is usually obtained via some kind of training procedure, and thus it could be a function of $\bx_S$. Next, we partition both $\bz=[ \bv ~~ \bx_S ]^\top$ and  $\bd_z=[\bd_v ~ \bd_{S} ]^\top$. Moreover, we partition $g(\bv, \bx_S)=[ g_{\bx_S}(\bv,\bx_S) ~~ g_{\bx_{S^c}} (\bv,\bx_S) ]^\top$ $= [ \bx_S ~  \bx_{S^c} ]^\top$. Then, the matrix of derivatives can be partitioned as follows:
 \begin{equation*}
     \bJ_z^{(\bx)} = \begin{bmatrix} \bJ_\bv^{(\bx_{S^c})} & \bJ_{x_S}^{(\bx_{S^c})} \\ \bJ_{\bv}^{(\bx_S)} & \bJ_{\bx_S}^{(\bx_S)} \end{bmatrix} :=  \begin{bmatrix} \bA & \bB \\ \bC & \bD \end{bmatrix}.
 \end{equation*}
 Since we are not interested in applied changes to $\bv$ we set $\bd_v{:=}\mathbf{0}$. By Lemma \ref{lemma:recourse_cost_general} we know $ \lVert \bd_x \rVert^2 {=}\bd^\top_z \big({\bJ_z^{(\bx)}}^\top \bJ_\bz^{(\bx)}\big) \bd_z$. A direct computation with $\bd_z {:=} \begin{bmatrix} \mathbf{0} & \bd_{S} \end{bmatrix}^\top$  yields:
 \begin{align*}
     \lVert \bd_x \rVert^2 &\approx \begin{bmatrix} \mathbf{0} & \bd_{S} \end{bmatrix} \begin{bmatrix} \bA & \bC \\ \bB & \bD \end{bmatrix} \begin{bmatrix} \bA & \bB \\ \bC & \bD \end{bmatrix} \begin{bmatrix} \mathbf{0} \\ \bd_{S} \end{bmatrix} \\
     & = \bd_{S}^\top \bB^\top \bB \bd_{S} + \bd_{S}^\top \bD^\top \bD \bd_{S} \\
     &=    \underbrace{\bd^\top_{S} \big({\bJ_{\bx_{S}}^{(\bx_{S^c})}}^\top \bJ_{\bx_S}^{(\bx_{S^c})}\big) \bd_{S}}_{\textcolor{BrickRed}{\text{Indirect Costs}}} + \underbrace{\bd^\top_{S} \big({\bJ_{\bx_S}^{(\bx_S)}}^\top \bJ_{\bx_S}^{(\bx_S)}\big) \bd_{S}}_{\textcolor{RoyalBlue}{\text{Direct Costs}}}.
\end{align*}
By the chain rule of multivariate calculus (recall that $\bv$ and $\bx_S$ need not be independent), note that we can write out the above terms as follows:
\begin{align*}
    {\bJ_{\bx_S}^{(\bx_{S^c})}} &= 
    %\frac{d g_{\bx_{S^c}}(\bv, \bx_S)}{d \bx_S} =
    \frac{\partial g_{\bx_{S^c}}(\bv, \bx_S)}{\partial \bv} \frac{\partial \bv}{\partial \bx_S} + \frac{\partial g_{\bx_{S^c}}(\bv, \bx_S)}{\partial \bx_S} \frac{\partial \bx_S}{\partial \bx_S} \\
    & = \underset{\textcolor{BrickRed}{\text{Entanglement costs}}}{\underbrace{\frac{\partial g_{\bx_{S^c}}(\bv, \bx_S)}{\partial \bv} \frac{\partial \bv}{\partial \bx_S}}} + \underset{\textcolor{BrickRed}{\text{Elasticity of $g{(\bx_{S^c})}$  w.r.t to $\bx_S$} }}{\underbrace{\frac{\partial g_{\bx_{S^c}}(\bv, \bx_S)}{\partial\bx_S}}} \\
    {\bJ_{\bx_S}^{(\bx_S)}} &= 
    %\frac{d g_{x_{S}}(\bv, \bx_S)}{d \bx_S} = 
    \frac{\partial g_{\bx_{S}}(\bv, \bx_S)}{\partial\bv} \frac{\partial\bv}{\partial\bx_S} + \frac{\partial g_{\bx_{S}}(\bv, \bx_S)}{\partial\bx_S} \frac{\partial \bx_S}{\partial\bx_S} \\
    &= \underset{\textcolor{RoyalBlue}{\text{Entanglement costs}}}{\underbrace{\frac{\partial g_{\bx_{S}}(\bv, \bx_S)}{\partial\bv} \frac{\partial\bv}{\partial\bx_S}}} + \underset{\textcolor{RoyalBlue}{\text{Identity Mapping}}}{\underbrace{\frac{\partial g_{\bx_{S}}(\bv, \bx_S)}{\partial\bx_S}}}.
   \tag*{\qed}
\end{align*}
%\end{proof}
 Let us consider what this implies intuitively. 
 For the direct costs, notice that $g$ would achieve the best reconstruction of $\bx_S$ by using the identify mapping. Recall, in Section \ref{section:marie_algorithm}, we suggested to use a \texttt{ResNet} component within the decoder to enforce this identity mapping during training of our autoencoder model. Hence, under perfect disentanglement the disentanglement costs are 0, and the $\bJ_{\bx_S}^{(\bx_S)}{=} \mathbf{1}$: thus, the direct cost would ideally be given by $\bd_{S}^{\top} \bd_{S}$. This is the squared $\ell_2$ norm of $\bd_{S}$. 
 
 The indirect costs, on the other hand, depend on the sensitivity of $\bx_{S^c}$ with respect to $\bx_S$, that is, $\bJ_{\bx_{S}}^{(\bx_{S^c})}$. Again, we consider the case of perfect disentanglement first: Suppose $\bx_S$ was a variable that was unrelated to the remaining variables $\bx_{S^c}$, while still being predictive of the outcome: Then $\bJ_{x_{S}}^{(x_{S^c})} = \mathbf{0}$, and a change $\bd_{S}$ would only have a direct impact on the outcome, and thus the indirect costs would disappear. In this case, the recourse cost for independence--based and dependence--based methods coincide. On the other extreme, suppose $\bx_{S}$ was almost a copy of $\bx_{S^c}$, then $\bJ_{\bx_{S}}^{(\bx_{S^c})} \approx \mathbf{1}$, and changing $\bx_S$ clearly impacts the remaining variables $\bx_{S^c}$. In this case, an independence--based method would not reliably capture the recourse costs. 

\subsection{Proof of Proposition \ref{proposition:dear}} \label{appendix:proof_closed_form_dear}

\begin{proof}[Proof of Proposition \ref{proposition:dear}]
Recall the problem in \eqref{equation:problem_dependent_partition}:
\begin{equation}
\bd_{\mathcal{S}}^* = \argmin_{\bd_{\mathcal{S}}} \mathcal{L} = \argmin_{\bd_{\mathcal{S}}} \lambda \lVert \bd_{\mathcal{S}} \rVert^2  + \lVert s - f\big(g(\bv, \bx_{\mathcal{S}} + \bd_{\mathcal{S}})\big)  \rVert^2.
\label{equation:objective_proof_dependent}
\end{equation}
We use the following first-order approximation to $f\big(g(\bv, \bx_{\mathcal{S}} + \bd_{\mathcal{S}})\big) \approx f(\bx) + \nabla f(\bx)^\top {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bd_{\mathcal{S}}$, where we have substituted $g(\bv, \bx_{\mathcal{S}}) = \bx$ and used that $\bv \upmodels \bx_{\mathcal{S}}$ by design of the generative model. Then, we can derive a surrogate loss to the loss from \eqref{equation:objective_proof_dependent}:
 \begin{align}
\mathcal{L} \approx \tilde{\mathcal{L}} = \lambda \cdot \bd_{\mathcal{S}}^\top \bd_{\mathcal{S}} +  \big(m - \nabla f(\bx)^\top {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bd_{\mathcal{S}} \big)^\top \big( m - \nabla f(\bx)^\top {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bd_{\mathcal{S}} \big),
\label{equation:surrogate_loss}
\end{align}
where $m = s - f(\bx)$.
The second term on the right in \eqref{equation:surrogate_loss} can be written as:
\begin{align*}
m^2 - 2 m \nabla f(\bx)^\top {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bd_{\mathcal{S}} + \bd_{\mathcal{S}}^\top  {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}^\top \nabla f(\bx) \nabla f(\bx)^\top  {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bd_{\mathcal{S}}.
\end{align*}
By solving $\argmin_{\bd_{\mathcal{S}}} \tilde{\mathcal{L}}$ we find the optimal change required in the features $\bx_{\mathcal{S}}$ as follows:
\begin{align}
    \tilde{\bd}_{\mathcal{S}}^* = \bm{M}^{-1}  \bm{\eta},
\end{align}
where
\begin{align}
\bm{M} & = \lambda \cdot \bI + {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}^\top \nabla f(\bx) \nabla f(\bx)^\top  {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}  &
\bm{\eta} & = m \cdot \nabla f(\bx)^\top {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}.
\label{eq:closed_form}
\end{align}
Next, we define $\bw = {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}^\top \nabla f(\bx)$. Note that $\bw \bw^\top$ is a rank-1 matrix. Thus, by the well-known Sherman-Morrison-Woodbury formula, $\bM$ can be inverted as follows:
\begin{align}
    \bM^{-1} = \frac{1}{\lambda} \bigg(\bI - \frac{\bw \bw^\top}{\lambda + \lVert \bw \rVert_2^2} \bigg).
\label{eq:inverse}
\end{align}
As a consequence, after substituting \eqref{eq:inverse} into \eqref{eq:closed_form} we obtain that:
\begin{align}
    \tilde{\bd}_{\mathcal{S}}^* = \frac{m}{\lambda + \lVert \bw \rVert_2^2} \bw.
\end{align}
Further, note that $\bdelta = g(\bz + \bd_{\mathcal{S}}) - g(\bz) \approx {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bd_{\mathcal{S}}$, where we have used that $\bv \upmodels \bx_{\mathcal{S}}$.
Therefore, we obtain a first-order approximation to the optimal recourse in input space:
\begin{align}
\bdelta^*_x \approx {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \tilde{\bd}_{\mathcal{S}}^* = \frac{m}{\lambda + \lVert \bw \rVert_2^2} \cdot {\bY_{\bx_{\mathcal{S}}}^{(\bx)}} \bw,
\label{eq:closed_form_explicit}
\end{align}
as claimed.
\end{proof}



\subsection{Proof of Lemma 1}
\begin{lemma}[Recourse costs in terms latent space quantities]
Given a latent representation $\bz$ of a sample $\bx=g(\bz)$ and a generated counterfactual $\xC=g(\zC)$ with $\zC = \bz + \bd_z$, the cost of recourse $\lVert \bx - \xC \rVert^2$ can be expressed in terms of latent space quantities:
\begin{align*}
 \lVert \bdelta_x \rVert^2
 &\approx   \bd^\top_z \big({\bJ_z^{(\bx)}}^\top \bJ_z^{(x)}\big) \bd_z ,
\end{align*}
where the matrix of derivatives with respect to output $\bx=g(\bz)$ is given by $\left.\bJ_z^{(\bx)}{:=} \frac{\partial g(\bz)}{\partial \bz }\right\vert_{\bz=\bz}$.
\label{lemma:recourse_cost_general}
\end{lemma}
\begin{proof}
We use the cost of recourse, and a first-order Taylor series approximation for $g(\bz+ \bd_z)$ at $\bz$ to arrive at:
\begin{align*}
\lVert \bdelta_x \rVert^2 &= \lVert g(\bz) -g(\bz + \bd_z) \rVert^2  \\
&\approx \lVert g(\bz) - (g(\bz)+{\bJ_\bz^{(\bx)}}\bd_z) \rVert^2  \\
 &= \bd^\top_z \big({\bJ_z^{(\bx)}}^\top \bJ_z^{(\bx)}\big) \bd_z,
\end{align*}
where $\left.\bJ_\bz^{(\bx)} := \frac{\partial g(\bz) }{\partial \bz }\right\vert_{\bz=\bz}$.
\end{proof}
On an intuitive level, Lemma \ref{lemma:recourse_cost_general} measures how the cost -- measured in input space quantities -- depends on perturbations of each component of the generative latent space $\bz$. 


% \section{Optimizing Our Objective} \label{section:marie_algorithm}
% Motivated by the insights from Propositions \ref{proposition:recourse_costs_ae} and \ref{proposition:dear}, we present an algorithmic procedure to compute minimal cost recourses under feature dependencies using a penalty term during autoencoder training that encourages disentanglement of $\bx_{\mathcal{S}}$ and $\bv$ in order to keep the \emph{entanglement costs} low.
% In summary, \texttt{DEAR} requires two steps: first, we need to obtain a latent space representation $\bv$, which is independent of $\bx_{\mathcal{S}}$. 
% Second, we require an optimization procedure to identify the nearest counterfactual.

% \begin{figure}[htb]
% \centering
% \begin{subfigure}[b]{0.49\columnwidth}
% \centering
% \input{tikz/training_time}
% \caption{Conditional autoencoder}        
% \label{fig:c_ae}
% \end{subfigure} 
% \hfill
% \begin{subfigure}[b]{0.49\columnwidth}
% \centering 
% \input{tikz/resnet}
% \caption{\texttt{ResNet} component within the decoder}
% \end{subfigure}
% \caption{\texttt{DEAR}'s autoencoder architecture.
% In (a), we show our conditional autoencoder architecture, which we train subject to the Hessian penalty described in Section \ref{section:marie_algorithm}. 
% In (b), we show how we achieve the identity mapping between $\bx_{\mathcal{S}}$ and the reconstructed $\bx^r_{\mathcal{S}}$ using a \texttt{ResNet} component \citep{he2016deep,he2016identity}: we add $\bx_{\mathcal{S}}$ to $\bx^r_{\mathcal{S}}$  before passing the arguments to the loss $\mathcal{L}_R$ from \eqref{eq:reconstruction_loss}.}
% \label{figure:architecture}
% \end{figure}

% \paragraph{\textbf{Step 1: Training the Generative Model}}
% The main idea is to train a generative model, in which $\bx_{\mathcal{S}}$ is independent of the latent variable $\bv$, while providing high-quality reconstruction of the input $\bx$.
% Thus, the training loss for the generative model consists of two components. 
% First, it consists of both an encoder network $e$ and decoder network $g$, for which the reconstruction loss,
% \begin{align}
% \mathcal{L}_R(g,e; \bx_{\mathcal{S}}) =\lVert g( e(\bx), \bx_{\mathcal{S}}) - \bx \rVert_2^2,
% \label{eq:reconstruction_loss}
% \end{align}
% guides both networks towards a good reconstruction of $\bx$.
% Second, we want to drive the \emph{entanglement costs} to 0, for which we need the decoder $g$ to be disentangled with respect to the latent space, i.e., each component of $\bz = [\bv, \bx_{\mathcal{S}}]$ should ideally control a single factor of variation in the output of $g$. 
% To formalize this intuition, recall that $g(\bx_{\mathcal{S}}, \bv) = \bx \in \mathbb{R}^d$, where each output $g_j=x_j$ for $1 \leq j \leq d$ has its own $|\bx_{\mathcal{S}}| \times |\bv|$ Hessian matrix $\bH^{(j)}$. 
% We refer to the collections of the $d$ Hessian matrices as $\bH$.
% Thus, the second loss we seek to minimize is given by:
% \begin{align}
%     \mathcal{L}_{\bH}(g; \bx_{\mathcal{S}}) = \sum_{j=1}^d \bigg( \sum_{k=1}^{|\bv|} \sum_{l=1}^{|\bx_{\mathcal{S}}|} H_{kl}^{(j)} \bigg),
% \label{eq:hessian_penalty}
% \end{align}
% which is also known as the Hessian penalty \citep{peebles2020hessian}.
% We illustrate the intuition of this objective on the $j$-th output $x_j$: we regularize the Hessian matrix $\bH^{(j)} = \frac{\partial}{\partial \bv} \frac{\partial g_j}{\partial \bx_{\mathcal{S}}}$ and encourage its off-diagonal terms to become $0$. 
% Driving the off-diagonal terms to $0$ implies that $\frac{\partial g_j}{\partial \bx_{\mathcal{S}}}$ is not a function of $\bv$ and thus $\bv$ plays no role for the output of $g_j$ when searching for minimum cost actions using $\bx_{\mathcal{S}}$.
% We use the Hessian penalty from \citep{peebles2020hessian} in our implementation.
% %Third, to keep the cost of recourse low we use the $\ell_1$-norm of the jacobian as a regularizer, i.e., we add $\lVert {\bY_{\bx_{\mathcal{S}}}^{(\bx)}}\rVert_1$ to the loss.
% Finally, Proposition \ref{proposition:recourse_costs_ae} requires the identity mapping between the latent space $\bx_{\mathcal{S}}$ and the reconstructed $\bx^r_{\mathcal{S}}$.
% We encourage our generator $g$ to learn this mapping by using a \texttt{ResNet} architecture \citep{he2016deep,he2016identity} as shown in Figure \ref{figure:architecture}.

% \paragraph{\textbf{Step 2: Finding Minimal Cost Actions $\bd_{\mathcal{S}}$}} Given our trained generative model from step 1, we rewrite the problem in \eqref{equation:problem_dependent_partition} using a Lagrangian with trade-off parameter $\lambda$. 
% For a given encoded input instance $e(\bx) = [\bv, \bx_{\mathcal{S}}]$, our objective function reads:
% \begin{align}
%      \bd^*_{\mathcal{S}} = \argmin_{\bd_{\mathcal{S}}, ~ \xC \in \mathcal{A}_d} \mathcal{L}  = \argmin_{\bd_{\mathcal{S}}, ~ \xC \in \mathcal{A}_d} \ell\big(f(\xC(\bd_{\mathcal{S}})), s \big) + \lambda \lVert \bx - \xC(\bd_{\mathcal{S}}) \lVert_1 ,
% \label{equation:surrogate_loss_dear}
% \end{align}
% where $\xC(\bd_{\mathcal{S}}) = g(\bv, \bx_{\mathcal{S}}+\bd_{\mathcal{S}})$ is a potential counterfactual in input space, $\ell(\cdot, \cdot)$ denotes the MSE loss, and $s\geq0$ is the target score in logit space. 
% % The MSE loss encourages the model output $f(\xC(\bd_{\mathcal{S}}))$ to be pushed to the target logit score $s$. 
% The term on the right side encourages the counterfactual $g(\bv, \bx_{\mathcal{S}}+\bd_{\mathcal{S}}) = \xC$ to be close to the given input point $\bx$, while the left hand side encourages the predictions to be pushed from the factual output $f(\bx)$ towards s. 
% We do gradient descent iteratively on the loss function in \eqref{equation:surrogate_loss_dear} until the class label changes from $y=0$ to $y=1$.
% Algorithm \ref{algorithm:dear_differentiable} summarizes our optimization procedure.
% Below we further discuss how other constraints can be included into our objective.
% \begin{algorithm}[tb]
%   \caption{\texttt{DEAR}}
%   \label{alg:example}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} $f$, $\bx$ s.t.\ $f(\bx){<}0$, $g$, $e$, $\lambda> 0$, Learning rate: $\alpha>0$, $s\geq 0$, $\mathcal{S}$
%   \STATE {\bfseries Initialize:} $\bd_{\mathcal{S}} = \mathbf{0}$, $ e(\bx)=[\bv, \bx_{\mathcal{S}}]$, $\xC = g(\bv, \bx_{\mathcal{S}} + \bd_{\mathcal{S}})$
%   \WHILE{$f(\xC)< s$} 
%   \STATE $\bd_{\mathcal{S}} =  \bd_{\mathcal{S}} - \alpha \cdot \nabla_{\bd_{\mathcal{S}}} \mathcal{L}(\xC(\bd_{\mathcal{S}});f, s, \lambda)$ \COMMENT{Optimize
%   \eqref{equation:surrogate_loss_dear}}
%   \STATE $\xC = g(\bv, \bx_{\mathcal{S}}+\bd_{\mathcal{S}})$
%   \ENDWHILE ~ \COMMENT{Class changed, i.e., $f(\xC) \geq s$}
%   \STATE {\bfseries Return:} $\xC^* = \xC$ 
% \end{algorithmic}
% \label{algorithm:dear_differentiable}
% \end{algorithm}

% \section{Experimental Results} \label{section:experiments}
% \input{sec5_iclr}

\section{Implementation Details} \label{Appendix:architecture_params}

%\subsection{Implementation Details}
%For all data sets, categorical features are binary encoded and data is scaled to lie between $0$ and $1$. We partition the data sets into train-test splits. The training set is used to train the classification models for which algorithmic recourse is generated. 
%For recourse methods, all features are assumed actionable for comparison to ensure fair comparison across methods.

%\subsection{Supervised Classification Models}
%All models are implemented in PyTorch 
%or TensorFlow 
%and use a $80-20$ train-test split for model training and evaluation. We evaluate model quality based on the model accuracy. All models are trained with the same architectures across the data sets:


\subsection{Recourse Methods}
For all data sets, the features are binary-encoded and the data is scaled to lie between $0$ and $1$. 
We partition the data sets into train-test splits. The training set is used to train the classification models for which recourses are generated.
Recourses are generated for all samples in the test split for the fixed classification model. 
In particular, we use the following algorithms to generate recourses. Specifically,
\begin{itemize}
\item \underline{{\texttt{SCFE}}} As suggested in~\citet{wachter2017counterfactual}, an Adam optimizer is used to oprimize \eqref{equation:problem_independent}. 
We obtain recourses using an $\ell_1$ distance function, and the binary cross entropy loss between the counterfactual label and the target. 

\item \underline{{\texttt{GS}}}
The explanation model uses a counterfactual search algorithm in the input space. 
Particularly, instances are sampled within an $\ell_1$-norm ball with search radius search radius $r_i$ until recourse is successfully obtained.
The search radius of the norm ball is increased until recourse is found. 

\item \underline{{\texttt{C-CHVAE}}} An autoencoder is additionally trained to model the data-manifold. 
The explanation model uses a counterfactual search algorithm in the latent space of the AE. 
Particularly, a latent sample within an $\ell_1$-norm ball with search radius $r_l$ is used until recourse is successfully obtained. 
The search radius of the norm ball is increased until recourse is found. 
The architecture of the generative model are provided in Appendix~\ref{app:vae_architecture}.

\item \underline{{\texttt{REVISE}}} As with the recourse model of \citet{pawelczyk2019}, an autoencoder is additionally trained to model the data-manifold. The explanation model uses a gradient-based search algorithm in the latent space of the AE.
For a fixed weight on the distance component, we allow up to 500 gradient steps until recourse is successfully obtained.
Moreover, we iteratively search for the weight leading up to minimum cost recourse. 
The architectures of the generative model are provided in Appendix~\ref{app:vae_architecture}.
\end{itemize}

We describe architecture and training details in the following.

\subsection{Supervised Classification Models}

All models are implemented in PyTorch and use a $80-20$ train-test split for model training and evaluation. We evaluate model quality based on the model accuracy. All models are trained with the same architectures across the data sets:

\begin{table}[h!]
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
                         & Neural Network                       & Logistic Regression        \\ \midrule
Units                    & [Input dim, 18, 9, 3, 1] & [Input dim, 1] \\
Type                     & Fully connected                      & Fully connected            \\
Intermediate activations & ReLU                                & N/A                        \\
Last layer activations   & Sigmoid                              & Sigmoid                    \\ \bottomrule
\end{tabular}
%}
\caption{Classification Model Details}
\label{tab:model_details}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{@{}l|llll@{}}
\toprule
              &                                                               & Adult & COMPAS & Give Me Credit \\ \midrule
Batch-size    & ANN                                                            & 512   & 32     & 64            \\ \cmidrule(l){2-5} 
              & \begin{tabular}[c]{@{}l@{}}Logistic\\ Regression\end{tabular} & 512   & 32     & 64            \\ \midrule
Epochs        & ANN                                                            & 50    & 40     & 30            \\ \cmidrule(l){2-5} 
              & \begin{tabular}[c]{@{}l@{}}Logistic\\ Regression\end{tabular} & 50    & 40     & 30            \\ \midrule
Learning rate & ANN                                                            & 0.002 & 0.002  & 0.001         \\ \cmidrule(l){2-5} 
              & \begin{tabular}[c]{@{}l@{}}Logistic\\ Regression\end{tabular} & 0.002 & 0.002  & 0.001         \\ \bottomrule
\end{tabular}
\caption{Training details}
\label{tab:train_dets}
\end{table}

{\begin{table}[h!]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
 & Adult & COMPAS & Give Me Credit \\ \midrule
Logistic Regression & 0.83  & 0.84  & 0.92  \\
Neural Network & 0.84  & 0.85  & 0.93  \\ \bottomrule
\end{tabular}
\caption{Performance of classification models used for generating algorithmic recourse.}
\label{tab:classifier_acc}
\end{table}
}


\subsection{Generative Model Architectures used for \texttt{DEAR}, \texttt{CCHVAE} and \texttt{REVISE}}\label{app:vae_architecture}
For all experiments, we use the following architectures.

\begin{table}[h!]
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
& Adult                      & COMPAS  & Give Me Credit      \\ \midrule
Encoder layers                 & [input dim, 16, 32, 10] & [input dim, 8, 10, 5] & [input dim, 8, 10, 5]  \\
Decoder layers                  & [10, 16, 32, input dim] & [5, 10, 8, input dim] & [5, 10, 8, input dim] \\
Type                     & Fully connected                      & Fully connected & Fully connected \\
% activations & ReLU                                & ReLU      & ReLU                  \\
Loss function   & MSE                             & MSE  & MSE                 \\ \bottomrule
\end{tabular}
%}
\caption{Autoencoder details}
\label{tab:autoencoder_dets}
\end{table}


Additionally, for \texttt{DEAR} all generative models use the Hessian Penalty \citep{peebles2020hessian} and a residual block, which we both described in more detail in Section \ref{section:marie_algorithm} of the main text.


% \subsection{Monotonicity Constraints}
% We set the following monotonicity constraints. The arrows indicate in which direction we allow the features to move. The constraints are added using the hinge-losses as described in Section \ref{section:marie_algorithm}. For every feature, we have assigned weights which we denoted by $\lambda_i$. Note that running our algorithm in an unconstrained fashion will lead to lower recourse costs.
% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%          Feature & Up/Down & Weight  \\
%          \midrule
%          \texttt{Age} & $\uparrow$ & 0.2 \\
%          \texttt{Educ} & $\uparrow$  & 0.05 \\
%          \texttt{C-gain} & $\uparrow$  & 0.05 \\
%          \texttt{Hours} & $\uparrow$  & 0.05 \\
%          \texttt{C-loss} & $\downarrow$  & 0.35 \\
%          \texttt{W-class} & NA & NA \\
%          \texttt{M-status} & NA & NA \\
%          \texttt{Occu} & NA & NA \\
%          \texttt{Relation} & NA & NA \\
%          \texttt{Native} & NA & NA \\
%     \bottomrule
%     \end{tabular}
%     \caption{Monotonicity constraints on the adult data set}
%     \label{tab:mono_adult}
% \end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%          Feature & Up/Down & Weight  \\
%          \midrule
%          \texttt{Age} & $\uparrow$ & 0.2 \\
%          \texttt{j-fel} & $\downarrow$  & 0.05 \\
%          \texttt{d-score} & $\downarrow$  & 0.05 \\
%          \texttt{j-misc} & $\downarrow$  & 0.05 \\
%          \texttt{priors} & $\downarrow$  & 0.05 \\
%          \texttt{j-fel} & $\downarrow$  & 0.05 \\
%          \texttt{d-score} & $\downarrow$  & 0.05 \\
%          \texttt{j-misc} & $\downarrow$  & 0.05 \\
%          \texttt{priors} & $\downarrow$  & 0.05 \\
%          \texttt{c-jail} & $\downarrow$  & 0.05 \\
%          \texttt{r-jail} & $\downarrow$  & 0.05 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Monotonicity constraints on the COMPAS data set}
%     \label{tab:mono_compas}
% \end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%          Feature & Up/Down & Weight  \\
%          \midrule
%          \texttt{Age} & $\uparrow$ & 0.2 \\
%          \texttt{RevU} & $\downarrow$  & 0.15 \\
%          \texttt{30-59Late} & $\downarrow$  & 0.10 \\
%          \texttt{60-89Late} & $\downarrow$  & 0.10 \\
%          \texttt{90Late} & $\downarrow$  & 0.10 \\
%          \texttt{Income} & $\uparrow$  & 0.05 \\
%          \texttt{OpenL} & $\downarrow$  & 0.05 \\
%          \texttt{EstateL} & $\downarrow$  & 0.05 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Monotonicity constraints on the GMC data set}
%     \label{tab:mono_gmc}
% \end{table}

